Multi-Head Self-Attention via Vision Transformer for Zero-Shot Learning

Zero-Shot Learning (ZSL) aims to recognise unseen object classes, which are not observed during the training phase. The existing body of works on ZSL mostly relies on pretrained visual features and lacks the explicit attribute localisation mechanism on images. In this work, we propose an attention-based model in the problem settings of ZSL to learn attributes useful for unseen class recognition. Our method uses an attention mechanism adapted from Vision Transformer to capture and learn discriminative attributes by splitting images into small patches. We conduct experiments on three popular ZSL benchmarks (i.e., AWA2, CUB and SUN) and set new state-of-the-art harmonic mean results {on all the three datasets}, which illustrate the effectiveness of our proposed method.

==> reference.tex <==
@ARTICLE{8413121, 
author={Xian, Yongqin and Lampert, Christoph H. and Schiele, Bernt and Akata, Zeynep},  journal={IEEE TPAMI},   title={Zero-Shot Learning—A Comprehensive Evaluation of the Good, the Bad and the Ugly},   year={2019}}

%%%%%%%%%%%%%%%%%%
@INPROCEEDINGS{5206594,  author={Lampert, Christoph H. and Nickisch, Hannes and Harmeling, Stefan},  booktitle={CVPR},   title={Learning to detect unseen object classes by between-class attribute transfer},   year={2009}}


@inproceedings{Mikolov2013DistributedRO,
  title={Distributed Representations of Words and Phrases and their Compositionality},
  author={Tomas Mikolov and Ilya Sutskever and Kai Chen and G. Corrado and J. Dean},
  booktitle={NIPS},
  year={2013}
}


@inproceedings{ASbddad233,
title = "Describing objects by their attributes",
author = "Ali Farhadi and Ian Endres and Derek Hoiem and David Forsyth",
year = "2009",
series = "CVPRW",
}



@inproceedings{Pennington2014GloveGV,
  title={Glove: Global Vectors for Word Representation},
  author={Jeffrey Pennington and R. Socher and Christopher D. Manning},
  booktitle={EMNLP},
  year={2014}
}

@article{19748,
author = {Miller, George A.},
title = {WordNet: A Lexical Database for English},
year = {1995},
issue_date = {Nov. 1995},
publisher = {Association for Computing Machinery},
journal = {Commun. ACM},
}



@InProceedings{romera-paredes15,
  title = 	 {An embarrassingly simple approach to zero-shot learning},
  author = 	 {Romera-Paredes, Bernardino and Torr, Philip},
  booktitle = {ICML},
  year = {2015}
}


@InProceedings{AWA2:journals/corr/XianSA17,
  author    = {Yongqin Xian and
               Bernt Schiele and
               Zeynep Akata},
  title     = {Zero-Shot Learning - The Good, the Bad and the Ugly},
  booktitle   = {CVPR},
  year      = {2017}
}

@ARTICLE{AWA1:6571196,  author={Lampert, Christoph H. and Nickisch, Hannes and Harmeling, Stefan},  journal={IEEE TPAMI},   title={Attribute-Based Classification for Zero-Shot Visual Object Categorization},   year={2014}}




@techreport{CUB,
	Title = {{The Caltech-UCSD Birds-200-2011 Dataset}},
	Author = {Wah, C. and Branson, S. and Welinder, P. and Perona, P. and Belongie, S.},
	Year = {2011},
	Institution = {California Institute of Technology},
}

@INPROCEEDINGS{SUN,  author={G. {Patterson} and J. {Hays}},  booktitle={CVPR},   title={SUN attribute database: Discovering, annotating, and recognizing scene attributes},   year={2012}}



@inproceedings{Transfomer,
 author = {Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, \L ukasz and Polosukhin, Illia},
 booktitle = {NIPS},
 publisher = {Curran Associates, Inc.},
 title = {Attention is All you Need},
 year = {2017}
}


@InProceedings{NEURIPS2020_1457c0d6,
  title={Language models are few-shot learners},
  author={Brown, Tom B and Mann, Benjamin and Ryder, Nick and Subbiah, Melanie and Kaplan, Jared and Dhariwal, Prafulla and Neelakantan, Arvind and Shyam, Pranav and Sastry, Girish and Askell, Amanda and others},
  booktitle={NeurIPS},
  year={2020}
}



@article{Radford2019LanguageMA,
  title={Language Models are Unsupervised Multitask Learners},
  author={Alec Radford and Jeffrey Wu and R. Child and David Luan and Dario Amodei and Ilya Sutskever},
  year={2019}
}


@article{CrossViT,
  title={CrossViT: Cross-Attention Multi-Scale Vision Transformer for Image Classification},
  author={Chun-Fu Chen and Quanfu Fan and R. Panda},
  journal={arXiv},
  year={2021}
 }

@inproceedings{ViT,
title={An Image is Worth 16x16 Words: Transformers for Image Recognition at Scale},
author={Alexey Dosovitskiy and Lucas Beyer and Alexander Kolesnikov and Dirk Weissenborn and Xiaohua Zhai and Thomas Unterthiner and Mostafa Dehghani and Matthias Minderer and Georg Heigold and Sylvain Gelly and Jakob Uszkoreit and Neil Houlsby},
booktitle={ICLR},
year={2021}
}



@article{Touvron2020TrainingDI,
  title={Training data-efficient image transformers & distillation through attention},
  author={Hugo Touvron and M. Cord and M. Douze and Francisco Massa and Alexandre Sablayrolles and Herv'e J'egou},
  journal={arXiv},
  year={2020}
}


@article{DBLP:journals/corr/abs-2102-05644,
  author    = {Alaaeldin El{-}Nouby and
               Natalia Neverova and
               Ivan Laptev and
               Herv{\'{e}} J{\'{e}}gou},
  title     = {Training Vision Transformers for Image Retrieval},
  journal   = {arXiv},
  year      = {2021}
}

@article{khan2021transformers,
  title={Transformers in Vision: A Survey},
  author={Salman Khan and Muzammal Naseer and Munawar Hayat and Syed Waqas Zamir and F. Khan and M. Shah},
  journal={arXiv},
  year={2021}
}


@inproceedings{Lampert2009LearningTD,
  title={Learning to detect unseen object classes by between-class attribute transfer},
  author={Christoph H. Lampert and H. Nickisch and S. Harmeling},
  journal={CVPR},
  year={2009}
}


@inproceedings{AlHalah2016RecoveringTM,
  title={Recovering the Missing Link: Predicting Class-Attribute Associations for Unsupervised Zero-Shot Learning},
  author={Ziad Al-Halah and Makarand Tapaswi and R. Stiefelhagen},
  journal={CVPR},
  year={2016}}


@inproceedings{ConSE,
  title={Zero-Shot Learning by Convex Combination of Semantic Embeddings},
  author={Mohammad Norouzi and Tomas Mikolov and S. Bengio and Y. Singer and Jonathon Shlens and Andrea Frome and G. Corrado and J. Dean},
  booktitle={ICLR},
  year={2014}
}


@inproceedings{NIPS2011_5dd9db5e,
 author = {Ordonez, Vicente and Kulkarni, Girish and Berg, Tamara},
 booktitle = {NIPS},
 title = {Im2Text: Describing Images Using 1 Million Captioned Photographs},
 year = {2011}
}




@ARTICLE{9354184,  author={Fang, Yuchun and Xiao, Zhengye and Zhang, Wei and Huang, Yan and Wang, Liang and Boujemaa, Nozha and Geman, Donald},  journal={IEEE TIFS},   title={Attribute Prototype Learning for Interactive Face Retrieval},   year={2021}}


@article{DBLP:journals/corr/RosenfeldU16b,
  author    = {Amir Rosenfeld and
               Shimon Ullman},
  title     = {Action Classification via Concepts and Attributes},
  journal   = {arXiv},
  year      = {2016}
}


@article{DBLP:journals/corr/abs-1811-04309,
  author    = {Soubarna Banik and
               Mikko Lauri and
               Simone Frintrop},
  title     = {Multi-label Object Attribute Classification using a Convolutional
               Neural Network},
  journal   = {arXiv},
  year      = {2018}
}

@INPROCEEDINGS{8877393,  author={ul Hassan, Muneeb and Mulhem, Philippe and Pellerin, Denis and Quénot, Georges},  booktitle={CBMI},   title={Explaining Visual Classification using Attributes},   year={2019}}



@article{Liu2020ConvolutionalPL,
  title={Convolutional Prototype Learning for Zero-Shot Recognition},
  author={Zhizhe Liu and Xingxing Zhang and Zhenfeng Zhu and Shuai Zheng and Y. Zhao and Jian Cheng},
  journal={IVC},
  year={2020}
  
}


@ARTICLE{ALE,  author={Akata, Zeynep and Perronnin, Florent and Harchaoui, Zaid and Schmid, Cordelia},  journal={IEEE TPAMI},   title={Label-Embedding for Image Classification},   year={2016}}

@InProceedings{DAZLE,
author = {Huynh, Dat and Elhamifar, Ehsan},
title = {Fine-Grained Generalized Zero-Shot Learning via Dense Attribute-Based Attention},
booktitle = {CVPR},
year = {2020}
}


@InProceedings{10.1007/978-3-642-15555-0_10,
author="Yu, Xiaodong
and Aloimonos, Yiannis",
editor="Daniilidis, Kostas
and Maragos, Petros
and Paragios, Nikos",
title="Attribute-Based Transfer Learning for Object Categorization with Zero/One Training Example",
booktitle="ECCV",
year="2010"}



@InProceedings{Wang2009JointLO,
  title={Joint learning of visual attributes, object classes and visual saliency},
  author={G. Wang and D. Forsyth},
  booktitle={ICCV},
  year={2009}
}


@inproceedings{NIPS2009_1543843a,
 author = {Palatucci, Mark and Pomerleau, Dean and Hinton, Geoffrey E and Mitchell, Tom M},
 booktitle = {NIPS},
 title = {Zero-shot Learning with Semantic Output Codes},
 year = {2009}
}




@inproceedings{DeViSE,
 author = {Frome, Andrea and Corrado, Greg S and Shlens, Jon and Bengio, Samy and Dean, Jeff and Ranzato, Marc\textquotesingle Aurelio and Mikolov, Tomas},
 booktitle = {NIPS},
 title = {DeViSE: A Deep Visual-Semantic Embedding Model},
 year = {2013}
}




@article{DBLP:journals/corr/FuHXG15,
  author    = {Yanwei Fu and
               Timothy M. Hospedales and
               Tao Xiang and
               Shaogang Gong},
  title     = {Transductive Multi-view Zero-Shot Learning},
  journal   = {arXiv},
  year      = {2015},
  }




@article{10.1145/1007730.1007736,
author = {Guo, Hongyu and Viktor, Herna L.},
title = {Learning from Imbalanced Data Sets with Boosting and Data Generation: The DataBoost-IM Approach},
year = {2004},
publisher = {Association for Computing Machinery},
journal = {SIGKDD Explor. Newsl.}
}


@InProceedings{Xian2019FVAEGAND2AF,
  title={F-VAEGAN-D2: A Feature Generating Framework for Any-Shot Learning},
  author={Yongqin Xian and Saurabh Sharma and B. Schiele and Zeynep Akata},
  journal={CVPR},
  year={2019}
}

@INPROCEEDINGS{8578548,  author={Verma, Vinay Kumar and Arora, Gundeep and Mishra, Ashish and Rai, Piyush},  booktitle={CVPR},   title={Generalized Zero-Shot Learning via Synthesized Examples},   year={2018}}


@article{Schnfeld2019GeneralizedZA,
  title={Generalized Zero- and Few-Shot Learning via Aligned Variational Autoencoders},
  author={Edgar Sch{\"o}nfeld and Sayna Ebrahimi and Samarth Sinha and Trevor Darrell and Zeynep Akata},
  journal={CVPR},
  year={2019}
}



@INPROCEEDINGS {8578679,
author = {Y. Xian and T. Lorenz and B. Schiele and Z. Akata},
booktitle = {CVPR},
title = {Feature Generating Networks for Zero-Shot Learning},
year = {2018}
}



@INPROCEEDINGS{7780498,  author={Zhang, Han and Xu, Tao and Elhoseiny, Mohamed and Huang, Xiaolei and Zhang, Shaoting and Elgammal, Ahmed and Metaxas, Dimitris},  booktitle={CVPR},   title={SPDA-CNN: Unifying Semantic Part Detection and Abstraction for Fine-Grained Recognition},   year={2016}}



@InProceedings{He2016DeepRL,
  title={Deep Residual Learning for Image Recognition},
  author={Kaiming He and X. Zhang and Shaoqing Ren and Jian Sun},
  booktitle={CVPR},
  year={2016},
}



@article{Ren2015FasterRT,
  title={Faster R-CNN: Towards Real-Time Object Detection with Region Proposal Networks},
  author={Shaoqing Ren and Kaiming He and Ross B. Girshick and J. Sun},
  journal={IEEE TPAMI},
  year={2015}
}





@InProceedings{pmlr-v119-chen20s,
  title = 	 {Generative Pretraining From Pixels},
  author =       {Chen, Mark and Radford, Alec and Child, Rewon and Wu, Jeffrey and Jun, Heewoo and Luan, David and Sutskever, Ilya},
  booktitle = 	 {ICML},
  year = 	 {2020},
}



@inproceedings{APN,
 author = {Xu, Wenjia and Xian, Yongqin and Wang, Jiuniu and Schiele, Bernt and Akata, Zeynep},
 booktitle = {NIPS},
 title = {Attribute Prototype Network for Zero-Shot Learning},
 year = {2020}
}




@InProceedings{Gidaris2018DynamicFV,
  title={Dynamic Few-Shot Visual Learning Without Forgetting},
  author={Spyros Gidaris and Nikos Komodakis},
  booktitle={CVPR},
  year={2018}}




@INPROCEEDINGS{SSE,  author={Zhang, Ziming and Saligrama, Venkatesh},  booktitle={ICCV},   title={Zero-Shot Learning via Semantic Similarity Embedding},   year={2015}}



@INPROCEEDINGS{LATEM,
author={Xian, Yongqin and Akata, Zeynep and Sharma, Gaurav and Nguyen, Quynh and Hein, Matthias and Schiele, Bernt},  booktitle={CVPR},   title={Latent Embeddings for Zero-Shot Classification},   year={2016}}




@INPROCEEDINGS{SAE,
  title={Semantic Autoencoder for Zero-Shot Learning},
  author={Elyor Kodirov and Tao Xiang and S. Gong},
  booktitle={CVPR},
  year={2017}
}



@article{GAZSL:journals/corr/abs-1712-01381,
  author    = {Yizhe Zhu and
               Mohamed Elhoseiny and
               Bingchen Liu and
               Ahmed M. Elgammal},
  title     = {Imagine it for me: Generative Adversarial Approach for Zero-Shot Learning from Noisy Texts},
  journal   = {CVPR},
  year      = {2018}
}



@INPROCEEDINGS{DAZLE,  author={Huynh, Dat and Elhamifar, Ehsan},  booktitle={CVPR},   title={Fine-Grained Generalized Zero-Shot Learning via Dense Attribute-Based Attention},   year={2020}}




@INPROCEEDINGS{AREN,  author={Xie, Guo-Sen and Liu, Li and Jin, Xiaobo and Zhu, Fan and Zhang, Zheng and Qin, Jie and Yao, Yazhou and Shao, Ling},  booktitle={CVPR},   title={Attentive Region Embedding Network for Zero-Shot Learning},   year={2019}}



@inproceedings{ESZSL,
  title={An embarrassingly simple approach to zero-shot learning},
  author={B. Romera-Paredes and P. Torr},
  booktitle={ICML},
  year={2015}
}




@InProceedings{SJE,
  title={Evaluation of output embeddings for fine-grained image classification},
  author={Zeynep Akata and Scott E. Reed and D. Walter and H. Lee and B. Schiele},
  booktitle={CVPR},
  year={2015}
}



@article{GAZSL,
  title={Imagine it for me: Generative Adversarial Approach for Zero-Shot Learning from Noisy Texts},
  author={Yizhe Zhu and Mohamed Elhoseiny and Bingchen Liu and A. Elgammal},
  journal={arXiv},
  year={2017}
}


@INPROCEEDINGS {CLSWGAN,
author = {Y. Xian and T. Lorenz and B. Schiele and Z. Akata},
booktitle = {CVPR},
title = {Feature Generating Networks for Zero-Shot Learning},
year = {2018}
}



@InProceedings{f-VAEGAN-D2,
  title={F-VAEGAN-D2: A Feature Generating Framework for Any-Shot Learning},
  author={Yongqin Xian and Saurabh Sharma and B. Schiele and Zeynep Akata},
  journal={CVPR},
  year={2019}}



@inproceedings{SGMA,
 author = {Zhu, Yizhe and Xie, Jianwen and Tang, Zhiqiang and Peng, Xi and Elgammal, Ahmed},
 booktitle = {NIPS},
 title = {Semantic-Guided Multi-Attention Localization for Zero-Shot Learning},
 year = {2019}
}




@INPROCEEDINGS{Alamri,  author={Alamri, Faisal and Kalkan, Sinan and Pugeault, Nicolas},  booktitle={ICPR},   title={Transformer-Encoder Detector Module: Using Context to Improve Robustness to Adversarial Attacks on Object Detection},   year={2021}}




@INPROCEEDINGS{ImageNet,  author={Deng, Jia and Dong, Wei and Socher, Richard and Li, Li-Jia and Kai Li and Li Fei-Fei},  booktitle={CVPR},   title={ImageNet: A large-scale hierarchical image database},   year={2009}}



@article{Deep_transfomer,
  publtype={informal},
  author={Hugo Touvron and Matthieu Cord and Alexandre Sablayrolles and Gabriel Synnaeve and Hervé Jégou},
  title={Going deeper with Image Transformers},
  year={2021},
  journal={arXiv}
}

@article{Swin,
  author    = {Ze Liu and
               Yutong Lin and
               Yue Cao and
               Han Hu and
               Yixuan Wei and
               Zheng Zhang and
               Stephen Lin and
               Baining Guo},
  title     = {Swin Transformer: Hierarchical Vision Transformer using Shifted Windows},
  journal   = {arXiv},
  year      = {2021}
}


@article{TnT,
  author    = {Kai Han and
               An Xiao and
               Enhua Wu and
               Jianyuan Guo and
               Chunjing Xu and
               Yunhe Wang},
  title     = {Transformer in Transformer},
  journal   = {arXiv},
  year      = {2021}
  
}


@inproceedings{S2GA,
 author = {Yu, yunlong and Ji, Zhong and Fu, Yanwei and Guo, Jichang and Pang, Yanwei and Zhang, Zhongfei (Mark)},
 booktitle = {Advances in Neural Information Processing Systems},
 publisher = {Curran Associates, Inc.},
 title = {Stacked Semantics-Guided Attention Model for Fine-Grained Zero-Shot Learning},
 year = {2018}
}




@article{32933444718,
  title={A Survey of Zero-Shot Learning},
  author={W. Wang and V. Zheng and H. Yu and C. Miao},
  journal={ACM-TIST},
  year={2019}
}


@InProceedings{calibrated,
author="Chao, Wei-Lun
and Changpinyo, Soravit
and Gong, Boqing
and Sha, Fei",
editor="Leibe, Bastian
and Matas, Jiri
and Sebe, Nicu
and Welling, Max",
title="An Empirical Study and Analysis of Generalized Zero-Shot Learning for Object Recognition in the Wild",
booktitle="Computer Vision -- ECCV 2016",
year="2016"}


